On-the-fly Definition Augmentation of LLMs for Biomedical NER

Despite their general capabilities, LLMs still struggle on biomedical NER tasks, which are difficult due to the presence of specialized terminology and lack of training data. In this work we set out to improve LLM performance on biomedical NER in limited data settings via a new knowledge augmentation approach which incorporates definitions of relevant concepts on-the-fly. During this process, to provide a test bed for knowledge augmentation, we perform a comprehensive exploration of prompting strategies. Our experiments show that definition augmentation is useful for both open source and closed LLMs. For example, it leads to a relative improvement of 15\% (on average) in GPT-4 performance (F1) across all (six) of our test datasets. We conduct extensive ablations and analyses to demonstrate that our performance improvements stem from adding relevant definitional knowledge. We find that careful prompting strategies also improve LLM performance, allowing them to outperform fine-tuned language models in few-shot settings. To facilitate future research in this direction, we release our code at https://github.com/allenai/beacon.

==> 06_discussion.tex <==


\section{Discussion}
\label{sec:discussion}

\subsection{What categories of errors does definition knowledge help with?}
\label{ssec:qualdef}
To analyze which categories of errors definition augmentation helps with, we conduct a qualitative analysis of predictions from GPT-4 and Llama 2 for the same datasets that we ran ablations on (CDR and NCBI for GPT-4, CHIA and MEDM for Llama 2). For each dataset, we randomly sample 50 instances which contained one or more erroneous extractions in the zero-shot setting that were corrected via definition augmentation. For all instances, we qualitatively assess (i) whether corrections use information from provided definitions, and (ii) the type of error corrected. 

From our qualitative analysis, we find that for CDR and NCBI, 52 out of 59 and 58 out of 64 corrected entities respectively are fixed due to provided definition information. Similarly, for CHIA and MEDM, we observe that 71 out of 87 and 57 out of 89 entities respectively are corrected due to provided definitions. This assessment provides additional evidence that corrections are largely due to provided definitions. Across all datasets, type mismatch and boundary errors were the most common error types fixed using definition information.

% For LLama 2, we chose CHIA and MedM. 

% For CDR and NCBI, out of 59 corrected entities, 52 were corrected using provided definitions. 

% Similarly, for NCBI, out of 64 corrected entities, we quantify that 58 were corrected with the definitions provided. 

% which had one or more incorrect entities in zero shot without definition augmentation but were corrected when we provided definitions of the extracted entities and noun phrases. For GPT4, we used the same datasets which we did ablations on. 


\subsection{Does using strict F1 underestimate model performance?}
\label{ssec:humaneval}

As noted in \ref{sec:expframework}, we evaluate NER performance using strict F1. However, prior work has shown that strict metrics can underestimate the performance of generative models on information extraction tasks \cite{wadhwa2023revisiting}. Therefore, we conduct additional human evaluation to supplement our automated evaluation results. First, we determine whether strict evaluation underestimates performance on our datasets. We do this by sampling 20 instances containing extraction errors (according to strict F1) per dataset, and assessing whether those are actual errors or could potentially be considered valid entities. This preliminary analysis indicates that strict evaluation severely underestimates performance on PICO and CHIA, but not as much on other datasets. Therefore, we conduct a larger-scale human evaluation of predictions on these two datasets. For both datasets, we randomly sample 100 sentences containing erroneous extractions and re-assessed all false positive and false negative predictions. Table~\ref{tab:humnaeval} presents results from this evaluation, indicating that strict F1 underestimates performance on these two datasets by nearly 30\%-50\%. We defer the development of more flexible evaluation strategies for generative models on IE tasks to future work.

% Therefore, we have done a human evaluation on the “false positive” and “false negative” outputs produced by these models for 2 of these datasets which we determined with a preliminary human eval. 

\begin{table}[!h]
\centering
\small
\begin{tabular}{ lcc } 
\toprule
 \textbf{Setting} & \textbf{PICO} & \textbf{CHIA} \\
\midrule
 \textbf{\#FP/FN entities under strict F1} & 468 & 353 \\ 
 \textbf{\#Entities considered correct} & 243 & 103 \\ 
 \textbf{Percentage} & 51\% & 30\% \\
 \bottomrule
\end{tabular}
\caption{Number of errors in token level strict F1 which are corrected during human evaluation.}
\label{tab:humnaeval}
\end{table}
